A Strengthened Branch and Bound Algorithm for the Maximum Common (Connected) Subgraph Problem

We propose a new and strengthened Branch-and-Bound (BnB) algorithm for the maximum common (connected) induced subgraph problem based on two new operators, Long-Short Memory (LSM) and Leaf vertex Union Match (LUM). Given two graphs for which we search for the maximum common (connected) induced subgraph, the first operator of LSM maintains a score for the branching node using the short-term reward of each vertex of the first graph and the long-term reward of each vertex pair of the two graphs. In this way, the BnB process learns to reduce the search tree size significantly and improve the algorithm performance. The second operator of LUM further improves the performance by simultaneously matching the leaf vertices connected to the current matched vertices, and allows the algorithm to match multiple vertex pairs without affecting the solution optimality. We incorporate the two operators into the state-of-the-art BnB algorithm McSplit, and denote the resulting algorithm as McSplit+LL. Experiments show that McSplit+LL outperforms McSplit+RL, a more recent variant of McSplit using reinforcement learning that is superior than McSplit.

==> 03RW-old.tex <==
This section introduces the best-performing BnB algorithms for MCS, McSplit~\cite{MccreeshPT17} and McSplit+RL~\cite{liu2020learning}. 
To simplify the algorithm description, we initially assume that the graphs are undirected. And the method is easy to be adapted to handle various extensions of the problem~\cite{MccreeshPT17}. 

At each search node, the BnB algorithm first estimates an upper bound of the best solution that can be found in this subtree. If the upper bound is not larger than the size of the current best solution, that means a better solution cannot be found to update the current solution under this search node, so the algorithm prunes this branch and backtracks. Otherwise, the algorithm selects a new vertex pair to match, updates the current solution and then runs recursively. 
There are three %critical points
key issues for the BnB algorithm: 1) estimate the upper bound, 2) design heuristic branching strategy, 3) maintain candidate vertices of the two graphs. 
To address these key issues, McSplit and McSplit+RL propose label class and a learning based scoring mechanism for the branching nodes, respectively.

%In this section, we introduce the two best-performing BnB algorithms for MCS, McSplit~\cite{MccreeshPT17} and McSplit+RL~\cite{liu2020learning}. McSplit is the base version, which uses an elegant way to solve the above critical points. McSplit+RL proposes a learning based branching heuristic to improve the performance of McSplit, and is the state-of-the-art.

\subsection{McSplit} \label{Sec3.1}
\begin{algorithm}[tb]
\caption{MCS($D$, $\alpha$, $\beta$, $\gamma$, $S_{cur}$, $S_{best}$)}
\label{alg1}
\textbf{Input}: A bidomain list $D$; Three heuristic functions $\alpha$, $\beta$ and $\gamma$ of bidomain selecting, first vertex selecting and second vertex selecting respectively; the current maintain solution $S_{cur}$; the best record solution $S_{best}$.\\
\textbf{Output}: The optimal solution $S_{best}$.

\begin{algorithmic}[1] %[1] enables line numbers
\STATE $UB$ $\leftarrow$ overestimate($D$) $+$ $|S_{cur}|$
\IF {$UB \leq |S_{best}|$}
\STATE \textbf{return} $S_{best}$
\ENDIF
\STATE $\langle V_l, V_r \rangle$ $\leftarrow$ obtain a bidomain by the heuristic $\alpha(D)$
\STATE $p$ $\leftarrow$ obtain a vertex by the heuristic $\beta(V_l)$
\STATE $m$ $\leftarrow$ $|V_r|$
\FOR {i from 1 to $m$}
\STATE $q$ $\leftarrow$ obtain a vertex by the heuristic $\gamma(V_r, p)$
\STATE $V_r$ $\leftarrow$ $V_r \setminus \{q\}$
\STATE $L$ $\leftarrow$ obtain a matched vertex pair list of $\langle p, q \rangle$ 
\STATE $S_{cur}'$ $\leftarrow$ $S_{cur} \cup L$
\IF {$|S_{cur}'| > |S_{best}|$}
\STATE $S_{best}$ $\leftarrow$ $S_{cur}'$
\ENDIF
\STATE $D'$ $\leftarrow$ obtain a new bidomain list by maintaining $D$
\STATE $S_{best}$ $\leftarrow$ MCS($D'$, $\alpha$, $\beta$, $\gamma$, $S_{cur}'$, $S_{best}$)
\ENDFOR
\STATE $D'$ $\leftarrow$ obtain a new bidomain list by removing $p$ from $D$ 
\STATE $S_{best}$ $\leftarrow$ MCS($D'$, $\alpha$, $\beta$, $\gamma$, $S_{cur}$, $S_{best}$)
\STATE \textbf{return} $S_{best}$
\end{algorithmic}
\end{algorithm}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\columnwidth]{fig1.png}
\caption{ 
An example to illustrate the concepts of bidomain and label class for MCS. There are three matched vertex pairs $\langle 1, a \rangle$, $\langle 2, b \rangle$ and $\langle 3, c \rangle$. According to the definitions of bidomain and label class, the remaining vertices are partitioned into three valid bidomains $D$(``000'') $= \langle \{6\}, \{f\} \rangle$, $D$(``100'') $= \langle \{7, 8\}, \{d\} \rangle$ and $D$(``110'') $= \langle \{4\}, \{e\} \rangle$, etc, where ``0'' indicates that the vertex is not adjacent to the corresponding matched vertex and ``1'' otherwise.
%indicates the vertex is adjacent to the corresponding matched vertex. 
Note that $D$(``011'') and $D$(``111'') are invalid bidomains, as they cannot provide any matched vertex pair, and will be removed in the bidomain dividing process. 
}
\vspace{-1em}
\label{fig1}
\end{figure}

%Before discuss the algorithm, we first introduce two concepts of McSplit, called bidomain structure and label class.

Consider two undirected and unlabelling input graphs $G_0$ and $G_1$. The bidomain structure consists of two vertex sets $\langle V_l, V_r \rangle$, where $V_l$ and $V_r$ are subsets of $V(G_0)$ and $V(G_1)$ respectively. McSplit assigns a label to each of the vertices in the two input graphs that indicates the connectivity of the unmatched vertex and the matched vertices, and the label is represented by a ``01''-string. The vertices of two graphs have the same calss label are partitioned into a bidomain, therefore the two input graphs can be represented as a list of bidomains while the search process and 
any vertex pair selected from different vertex set is legal to match in each bidomain.
When a pair vertex $\langle p, q \rangle$ is matching, each bidomain $\langle V_l, V_r \rangle$ will divide into two new bidomains $\langle V_l^0, V_r^0 \rangle$ and $\langle V_l^1, V_r^1 \rangle$ where the superscript ``0'' and ``1'' indicate the connectivity of the matched vertex pair $\langle p, q \rangle$ and the new bidomains. The following example shows how the bidomain structure and label class work in the algorithm. 

\begin{example}
Figure~\ref{fig1} shows two undirected and unlabelling graphs $G_0$ and $G_1$. Initially, all vertices of the two graphs form a bidomain with an empty string label $D$(``'') $= \langle \{1, 2, 3, 4, 5, 6, 7, 8\}, \{a, b, c, d, e, f, g\} \rangle$. The first matched vertex pair is $\langle 1, a \rangle$, the bidomain $D$(``'') divides into $D$(``0'') $= \langle \{5, 6\}, \{f\} \rangle$ and $D$(``1'') $= \langle \{2, 3, 4, 7, 8\}, \{b, c, d, e, g\} \rangle$ where the vertices in the bidomain labelled by ``0'' are not adjacent to the vertices of matched pair and the vertices in the bidomain labelled by ``1'' are adjacent to one of the vertices of matched pair. 
Then the second matched vertex pair is $\langle 2, b \rangle$. Consequently, the bidomain $D$(``0'') divides into $D$(``00'') $= \langle \{6\}, \{f\} \rangle$ and $D$(``01'') $= \langle \{5\}, \emptyset \rangle$; the bidomain $D$(``1'') divides into $D$(``10'') $= \langle \{7, 8\}, \{d\}\rangle$ and $D$(``11'') $= \langle \{3, 4\}, \{c, e, g\} \rangle$. Note that the bidomain $D$(``01'') has an empty set that means it can not provide any matched vertex pair, therefore it is removed from the current bidomain list. After matching the third vertex pair $\langle 3, c \rangle$, the bidomains reaches a situation as shown in Figure~\ref{fig1}.
\end{example}

Obviously, a bidomain $\langle V_l, V_r \rangle$ can provide at most $\min (|V_l|, |V_r|)$ matched vertex pairs. Therefore, the algorithm estimates the upper bound of the list of bidomians $D$ by using the following equation:
\begin{equation} \label{eq1}
    OverEstimate(D) = \sum_{\langle V_l, V_r \rangle \in D} \min(|V_l|, |V_r|)
\end{equation}

Now, we introduce the flow of BnB algorithm based on the depth-first search for MCS, as depicted in Algorithm~\ref{alg1}. The call of MCS($\langle V(G_0), V(G_1) \rangle$, $\alpha$, $\beta$, $\gamma$, $\emptyset$, $\emptyset$) returns a maximum common subgraph of two input $G_0$ and $G_1$ where the $\alpha$, $\beta$ and $\gamma$ are the heuristics. 
At each search node, the algorithm calculates the upper bound assisted by Eq.~\ref{eq1} and it uses the upper bound to determine whether it can find better solution from this search node. If there does not exist a better solution from this node, the algorithm prunes and backtracks. 
Then the algorithm selects a bidomain $\langle V_l, V_r \rangle$ from the bidomain list by the heuristic $\alpha$ and picks a vertex $p$ from $V_l$ by heuristic $\gamma$. The algorithm enumerates all the vertices in $V_r$ to match  with the vertex $p$ where the order of enumeration is decided by the heuristic $\gamma$. When a vertex pair $\langle p, q \rangle$ is matched, the algorithm appends it to the current solution and updates the best solution, and obtains a new bidomain list by partitioning the current bidomain list by $\langle p, q \rangle$. Afterwards, the algorithm runs recursively with the new bidomain list. After enumerating all the possible matched vertex pair of $p$, the rest of situation is the vertex $p$ does not appear in the matched vertex pair list, thus the algorithm removes the vertex $p$ from the current bidomain list and runs recursively. 

The heuristic is the essential part in the BnB algorithm that decides the branching way of the search tree, the quality of heuristic will directly affects the search efficiency and the algorithm performance. 
There are three heuristics $\alpha$, $\beta$ and $\gamma$ appear in this BnB algorithm that represent the policy of selecting the bidomain, selecting the first matched vertex and the order of enumerating the second matched vertex respectively. 
The three heuristics of McSplit are shown as follows:
\begin{itemize}
\item $\alpha$: McSplit defines the value $\max(|V_l|, |V_r|)$ as the size of bidomain. It selects a bidomain with the smallest size from the bidomain list and uses the largest vertex degree in $V_l$ to break tie. By applying this policy, the algorithm will branch less at each search node and partitions the bidomains frequently. It certainly reduces the size of search tree. Notice it also can use the value $|V_l| \cdot |V_r|$ as the size of bidomain which means there are $|V_l| \cdot |V_r|$ ways to select a vertex pair from a bidomain, but the experimental result shows using $\max(|V_l|, |V_r|)$ is better. 
\item $\beta$: McSplit picks the largest degree vertex from $V_l$ as the first matched vertex. 
\item $\gamma$: McSplit enumerates the second matched vertex in $V_r$ with the order is the vertex degree from large to small.  
\end{itemize}

The selecting vertex pair heuristic $\beta$ and $\gamma$ of McSplit are naive and they are not adaptive. 

\subsection{McSplit+RL} 
Liu et al. propose a learning based branching heuristic to reduce the size of the BnB search tree inspired by reinforcement learning, they implement it on top of McSplit that obtains a new algorithm called McSplit~\cite{liu2020learning}. The goal of heuristic is hoping the algorithm to choice the branching with the largest bound reduction and reach the pruning condition as early as possible. They regard the BnB algorithm as an agent and selecting a vertex pair to match is an action. When a vertex pair $\langle p, q \rangle$ is matching, the current bidomain list $D$ divides into the new bidomian list $D'$, they use the esimating bound reduction of bidomain list as the reward $r(p, q)$ of taking the action $\langle p, q \rangle$, it can be formulated as follows:
\begin{equation} \label{eq2}
    r(p, q) = OverEstimate(D) - OverEstimate(D')
\end{equation}
Where the function $OverEstimate$ as shows in Equation~\ref{eq1}.

McSplit+RL maintains two score lists $S_0(\cdot)$ and $S_1(\cdot)$ for each vertex in $G_0$ and $G_1$, both lists are initialized to 0. At each search node, when the algorithm takes an action $\langle p, q \rangle$, McSplit+RL computes the reward $r(p, q)$ immediately and updates the score lists as follows:
\begin{equation}
\begin{aligned}
    S_0(p) &\gets S_0(p) + r(p, q) \\
    S_1(q) &\gets S_1(q) + r(p, q)
\end{aligned}
\end{equation}

McSplit+RL uses the two score lists to evaluate selecting which vertex can obtain the largest bound reduction. It replaces the heuristic $\beta$ and $\gamma$ in Section~\ref{Sec3.1} as follows:
\begin{itemize}
\item $\beta$: McSplit+RL picks the vertex $p$ with the largest score $S_0(p)$ from $V_l$ as the first matched vertex. 
\item $\gamma$: McSplit+RL enumerates the second matched vertex $q$ in $V_r$ with the order is the score $S_1(q)$ from large to small.  
\end{itemize}

Furthermore, McSplit+RL gives a variant algorithm called McSplit+RL$_{pair}$. It maintains a score list $S_0(\cdot)$ for each vertex in $G_0$ and a pair score list $S_{pair}(\cdot, \cdot)$ for each vertex pair in $V(G_0) \times V(G_1)$, both lists also are initialized to 0. The updating way is changed as follows:
\begin{equation}
\begin{aligned}
    S_0(p) &\gets S_0(p) + r(p, q) \\
    S_{pair}(p, q) &\gets S_{pair}(p, q) + r(p, q)
\end{aligned}
\end{equation}

The heuristic $\beta$ of McSplit+RL$_{pair}$ is still as same as McSplit+RL, and the heuristic $\gamma$ is changed as follows:
\begin{itemize}
\item $\gamma$: McSplit+RL enumerates the second matched vertex $q$ in $V_r$ with the order is the score $S_{pair}(p, q)$ from large to small.  
\end{itemize}

The experimental results~\cite{liu2020learning} show the performance of McSplit+RL is better. 
%Liu et al. proposed a heuristic branching strategy to reduce the size of search tree inspired by reinforcement. First, reward the vertices pair based on the reduction of UB. The vertices pair as branching node will effect the quality of subgraph. The more reduction of UB is, the more important the vertices are for induced subgraph. As Example 1 shows, $D$(``'') can provide seven vertices pairs on the future, but $D$(``0'') and $D$(``1'') provide at most $1 + 5 = 6$ matching pairs after choosing $\langle 1, a \rangle$. So, the matching action (vertex 1 and a) gets reward 0. McSplit+RL~\cite{liu2020learning} as an agent simply accumulates all actions rewards of each vertex as the vertex value. Second, the algorithm selects the vertex with maximum value from the pattern graph and target graph respectively, and breaks tie by vertex degree. Compared to the branching strategy based on vertex degree, the learning for branching node based on reinforcement finds the best solution as far as possible, and allows more diversified search.  




